Identification of Spikes in Time Series

Identification of unexpectedly high values in a time series is useful for epidemiologists, economists, and other social scientists interested in the effect of an exposure spike on an outcome variable. However, the best method to identify spikes in time series is not known. This paper aims to fill this gap by testing the performance of several spike detection methods in a simulation setting. We created simulations parameterized by monthly violence rates in nine California cities that represented different series features, and randomly inserted spikes into the series. We then compared the ability to detect spikes of the following methods: ARIMA modeling, Kalman filtering and smoothing, wavelet modeling with soft thresholding, and an iterative outlier detection method. We varied the magnitude of spikes from 10-50% of the mean rate over the study period and varied the number of spikes inserted from 1 to 10. We assessed performance of each method using sensitivity and specificity. The Kalman filtering and smoothing procedure had the best overall performance. We applied Kalman filtering and smoothing to the monthly violence rates in nine California cities and identified spikes in the rate over the 2005-2012 period.

==> Supplemental_Material.tex <==

rm(list = ls())
ls() 

library(tsoutliers) 
library(forecast)
library(KFAS)
library(wavethresh)
library(EbayesThresh)
library(TSA)
library(ggplot2)
library(RColorBrewer)
library(grid)


##########################################################################
            # Define functions for spike detection methods #
##########################################################################


####### ARIMA ####### 

ar.out <- function(ts,shocks) {
	
	arfit <- auto.arima(ts,allowdrift=T,allowmean=T) 
	resid <- residuals(arfit)

# locate shocks identified by procedure 
	idsh <- time(resid)[resid>2*sd(resid)]


# calculate relative frequency of correctly identifying outliers 
	rfreq <- mean(as.numeric(shocks %in% idsh))

# calculate average frequency of misidentifying outliers 
	afreq <- sum(as.numeric(!idsh %in% shocks))

	freq <- rbind(rfreq, afreq)
	#print("arima")
	#print(freq)
	return(freq)
	}
	
####### Kalman ####### 

kfs.out <- 	function(ts,shocks) {
	
    fit <- auto.arima(ts,allowdrift=T,allowmean=T) 	
	coef <- 	fit$coef

# get coefficients and order of differencing
	try(rm(ar))
		if (is.na(coef["ar1"])) ar <- NULL
		if (!is.na(coef["ar1"])) ar <- coef["ar1"]
		if (!is.na(coef["ar2"])) ar <- c(ar,coef["ar2"])
		if (!is.na(coef["ar3"])) ar <- c(ar,coef["ar3"])
		if (!is.na(coef["ar4"])) ar <- c(ar,coef["ar4"])
		if (!is.na(coef["ar5"])) ar <- c(ar,coef["ar5"])

try(rm(ma))
		if (is.na(coef["ma1"])) ma <- NULL
		if (!is.na(coef["ma1"])) ma <- coef["ma1"]
		if (!is.na(coef["ma2"])) ma <- c(ma,coef["ma2"])
		if (!is.na(coef["ma3"])) ma <- c(ma,coef["ma3"])
		if (!is.na(coef["ma4"])) ma <- c(ma,coef["ma4"])
		if (!is.na(coef["ma5"])) ma <- c(ma,coef["ma5"])


diff <- fit$arma[length(fit$arma)-1]

# fit Kalman filter and smoother
	model <- SSModel(ts ~ SSMarima(ar=ar,ma=ma,d=diff))
	fit <- fitSSM(model,inits=c(0,0))
	out.kfs <- KFS(fit$model)

# calculate residuals
resid <- ts - out.kfs$muhat 

# locate shocks identified by procedure 
	idsh <- time(resid)[resid>2*sd(resid)]

# calculate relative frequency of correctly identifying outliers 
	rfreq <- mean(as.numeric(shocks %in% idsh))

# calculate average frequency of misidentifying outliers 
	afreq <- sum(as.numeric(!idsh %in% shocks))

	freq <- rbind(rfreq, afreq)
	#print("kalman")
	#freq
	return(freq)
	
	}
	
####### Wavelets ####### 

s.wave.out <- function(ts,shocks) {

# apply wavelet transform and get coeffcients
	ws <- append(ts[1:96],rep(0,32))
	wmap <- wd(ws)
	smap <- threshold(wmap,type="soft",policy="universal")

	sfit <- wr(smap)
	
# calculate residuals	
	resid <- ws[1:96] - sfit[1:96]
		
# locate shocks identified by procedure 
try(rm(idsh))
	idsh <- time(resid)[resid>2*sd(resid)]


# calculate relative frequency of correctly identifying outliers 
try(rm(rfreq))
	rfreq <- mean(as.numeric(shocks %in% idsh))
	#print(rfreq)

# calculate average frequency of misidentifying outliers 
try(rm(afreq))
	afreq <- sum(as.numeric(!idsh %in% shocks))
	#print(afreq)

	freq <- rbind(rfreq, afreq)
	#print("wavelet, soft thresholding")
	#print(freq)
	return(freq)

}	

####### Outlier Detection ####### 

d.out <- function(ts,shocks) {
	
	arfit <- auto.arima(ts,allowdrift=T,allowmean=T) 
	dAO <- detectAO(arfit)
	
	
# locate shocks identified by procedure 
	idsh <- unique(dAO$ind[dAO$lambda2>0])


# calculate relative frequency of correctly identifying outliers 
	rfreq <- mean(as.numeric(shocks %in% idsh))

# calculate average frequency of misidentifying outliers 
	afreq <- sum(as.numeric(!idsh %in% shocks))

	freq <- rbind(rfreq, afreq)
	#print("arima")
	#print(freq)
	return(freq)
	}	
	
	

##########################################################################
                 # Define initial ARIMA models #
##########################################################################
set.seed(42654)

setwd("filepath")
source('./scripts/arima.R')
source("./scripts/tsoutliers.R")
source("./scripts/kfs.R")
source("./scripts/tsay.R")
source("./scripts/swavelet.R")
source("./scripts/hwavelet.R")
source("./scripts/ebt_wavelet.R")
source("./scripts/detectO.R")


# define iteration parameters
shock.num <- 1:10
shock.mag <- seq(0.1,0.5, by=0.1)

# Oakland parameters
oak.sim <-  function(iteration) arima.sim(n=96,list(order = c(4,1,2), ar = c(0.8481,-0.1436,0.3572,-0.6178), ma=c(-1.6616,0.7814)) , sd = c(0.0926, 0.1150,0.1129,0.0841,0.0812,0.0773,11.79155)) + 79.27858

# Richmond parameters
rich.sim <- function(iteration) arima.sim(n=96,list(order=c(0,1,1), ar = NULL, ma = c(-0.7940)),sd=c(0.0665, 12.49071)) + 73.68784

# Los Angeles parameters
la.sim <-  function(iteration) arima.sim(n=96,list(order=c(1,0,0),ar=c(0.436),ma=NULL), sd=c(0.093, 3.401935)) + 35.52811 

# Fresno parameters 
fres.sim <- function(iteration) arima.sim(n=96, list(order=c(1,1,1), ar=c(0.5306), ma=c(-0.9504)), sd=c(0.0966, 0.0319, 6.384975)) + 49.20486

# Sacramento parameters 
sac.sim <- function(iteration) arima.sim(n=96, list(order=c(2,0,1), ar=c(-0.465,0.5180), ma=c(0.9315)), sd=c(0.0938,0.0879, 0.0619, 6.854713)) + 50.98931 


# Berkeley parameters
berk.sim <- function(iteration) arima.sim(n=96, list(order=c(1,0,1), ar=c(0.8762), ma=c(-0.6531)), sd=c(0.1032, 0.1612, 6.836614)) + 28.40601 

# San Diego parameters
sd.sim <- function(iteration) arima.sim(n=96, list(order=c(2,0,0), ar=c(0.3605,0.1875), ma=NULL), sd=c(0.1003, 0.1018, 3.203321)) + 30.72144 

# SF paramaters
sf.sim <- function(iteration) arima.sim(n=96, list(order=c(1,0,0), ar=c(0.3151), ma=NULL), sd=c(0.0976,5.014734)) + 46.65183 

# Stockton parameters
stock.sim <- function(iteration) arima.sim(n=96, list(order=c(1,0,0), ar=c(0.3440), ma=NULL), sd=c(0.0978, 7.90195)) + 54.58181



# main function

shock.inner <- function(iteration,m,n,c) {
set.seed(iteration)
	
	
library(tsoutliers) 
library(forecast)
library(KFAS)
library(wavethresh)
library(EbayesThresh)

source('./scripts/arima.R')
source("./scripts/tsoutliers.R")
source("./scripts/kfs.R")
source("./scripts/tsay.R")
source("./scripts/swavelet.R")
source("./scripts/hwavelet.R")
source("./scripts/ebt_wavelet.R")
source("./scripts/detectO.R")

  # simulate time series 
  ts1 <- city[[c]](iteration)
  
  # print interation so you can track the simulation progress
  print(iteration)

  # randomly select n points to add shocks
  shocks <- sample(1:length(ts1), n, rep=F)
  
  # add shocks of size m
  ssize <- rep(m,length(shocks))
  
  tso <- ts1
  for (s in 1:length(shocks)) {	
    ts1[shocks[s]] <- ts1[shocks[s]]*(1+ssize[s]) 
  }
  
  
  ##########################################################################
                 # Measuring accuracy across methods #
  ##########################################################################
  
  ####### Arima #######
  arima <- ar.out(ts1, shocks) 

  
  ####### Kalman ######
  
  kalman <- kfs.out(ts1, shocks)


  ###### Wavelet ######
  swave <- s.wave.out(ts1, shocks)

  
  ###### Outlier detection ######
  detectO <- d.out(ts1,shocks)
	 
	 
  out <- cbind(arima,kalman,swave,detectO)
  return(out)
}


# Define city vector
city <- c(stock.sim, la.sim, oak.sim, rich.sim, fres.sim, sac.sim, berk.sim, sd.sim, sf.sim)
names(city) <- c("stock", "la", "oak", "rich", "fres", "sac", "berk", "sd", "sf")


############################## Run program for each city #############################


for (c  in 1:length(city)) {
  
  for  (n in shock.num ){
    for (m in shock.mag) {
    	
    print (paste("city =", names(city)[[c]],"n=",n,"m=",m))

    table <- lapply(1:1000, shock.inner,m=m,n=n,c=c)
   
  results <- na.omit(Reduce("+",table))
  colnames(results) <- c("Arima","Kalman","SoftWavelet","DetectO")
  

  write.csv(results, file = paste0("filepath",names(city)[[c]],"/results_",names(city)[[c]],"n",n,"m",m,".csv"))
    }
  }
}

##########################################################################
                 # Summarizing results #
##########################################################################


sensitivity <- list()
specificity <- list()

for (s in seq(10,60, by=10)) {
  sensitivity[[(s/10)]] <- data.frame(matrix(ncol=5, nrow=9))
  names(sensitivity[[(s/10)]]) <- c("City","Arima","Kalman","ST Wavelet","Detect AO")
  names(sensitivity)[[(s/10)]] <- paste0("sensitivity",s)
  
}

for (s in seq(10,60, by=10)) {
  specificity[[(s/10)]] <- data.frame(matrix(ncol=5, nrow=9))
  names(specificity[[(s/10)]]) <- c("City","Arima","Kalman","ST Wavelet","Detect AO")
  names(specificity)[[(s/10)]] <- paste0("specificity",s)
  
}

#### Read in csv files produced above and summarize 

for (c in 1:length(cities)) {
  
  city <- cities[c]
  
  df_r <- data.frame(matrix(ncol=6, nrow=50))
  df_a <- data.frame(matrix(ncol=6, nrow=50))
  
  colnames(df_r) <- c("Number","Magnitude","Arima","Kalman","ST Wavelet","Detect AO")
  colnames(df_a) <- c("Number","Magnitude","Arima","Kalman","ST Wavelet","Detect AO")
  
  for(n in 1:10) {
    for (m in 1:5) {
      df <- read.csv(paste0("./results/simulation output/",city,"/results_",city,"n",n,"m0.",m,".csv"))
      df_r[5*(n) + m - 5,1] <-n
      df_r[5*(n) + m - 5,2] <- m*10
      df_a[5*(n) + m - 5,1] <-n
      df_a[5*(n) + m - 5,2] <- m*10 
      for (i in 2:5) {
        df_r[5*(n) + m - 5,i+1] <- df[1,i]/10
        df_a[5*(n) + m - 5,i+1] <- 100*(96-n - df[2,i]/1000)/(96-n)
      }
    }
  }
  
  
  for (s in seq(10,60, by=10)) {

     if (s<=50) {
  sensitivity[[s/10]][c,] <- c(city,colMeans(df_r[df_r$Magnitude==s,])[3:6])
  specificity[[s/10]][c,] <- c(city,colMeans(df_a[df_a$Magnitude==s,])[3:6])
    }
    else {
    sensitivity[[s/10]][c,] <- c(city,colMeans(df_r)[3:6])
    specificity[[s/10]][c,] <- c(city,colMeans(df_a)[3:6])
     }
  write.csv(sensitivity[[s/10]],file=paste0("/Users/dana/Documents/Research Projects/Violence Shock Identification/results/tables/sensitivity",s,".csv"))
}



